Election Manipulation on Social Networks with Messages on Multiple Candidates

We study the problem of election control through social influence when the manipulator is allowed to use the locations that she acquired on the network for sending \emph{both} positive and negative messages on \emph{multiple} candidates, widely extending the previous results available in the literature that study the influence of a single message on a single candidate. In particular, we provide a tight characterization of the settings in which the maximum increase in the margin of victory can be efficiently approximated and of those in which any approximation turns out to be impossible. We also show that, in simple networks, a large class of algorithms, mainly including all approaches recently adopted for social-influence problems, fail to compute a bounded approximation even on very simple networks, as undirected graphs with every node having a degree at most two or directed trees. Finally, we investigate various extensions and generalizations of the model.

==> notation.tex <==


\begin{table}[!h]
	\small
	\centering
	%	\begin{tabular}{|l|l|}
	\renewcommand{\arraystretch}{1.5}
	
	\begin{tabular}{|c|c|c|c|c|}
		\hline
		&\textbf{standard} &  \textbf{bribed seeds} &  \textbf{pessimistic TBR} & \textbf{optimistic TBR} \\
		\hline 
		$+$, 3 candidates & $\notin$ \PolyAPX & $\notin$ \LogAPX & $\notin$ \PolyAPX & $\notin$ \PolyAPX\\ \hline
		
		$-$, 3 candidates & $\notin$ \PolyAPX & $\notin$ \LogAPX & $\notin$ \PolyAPX & $\mathsf{APX}$-Complete\\ \hline
		
		$\{+,-\}$, 3 candidates & $\mathsf{APX}$-Complete & $\mathsf{APX}$-Complete & $\notin$ \LogAPX & $\mathsf{APX}$-Complete \\ \hline
		
		$\{+,-\}$, 4 candidates & $\notin$ \PolyAPX  & $\notin$ \LogAPX & $\notin$ \LogAPX & $\notin$ \LogAPX\\ \hline  
	\end{tabular}
	\renewcommand{\arraystretch}{1}
	\caption[Variants' table]{Variants' table.}
	\label{tab:variants}
	
	
\end{table}

\begin{table}[!h]
	\small
	\centering
	%	\begin{tabular}{|l|l|}
	\renewcommand{\arraystretch}{1.5}
	
	\begin{tabular}{|l|l|}
		\hline
		\textbf{Symbol} &  \textbf{Meaning} \\
		\hline 
		$V$ & Set of vertices \\ \hline
		$E$ & Set of edges \\ \hline
		$G(V,E)$ & Graph \\ \hline
		$p(v,v' )$ & probability that edge exists \\ \hline
		$y$ & live-graph \\ \hline
		$S$ & Set of seeds \\ \hline
		$S^*$ & Optimal set of seeds of cardinality $k$\\ \hline
		$s$ & seed \\ \hline 
		$\pi_v$ & order of preferences of node $v$ \\ \hline
		$I(s)=(q_*,...,q_{|C|}), q \in \{-, \cdot,+\}$ & influences in a seed \\ \hline
		$\bar I(v)=(q_*,...,q_{|C|}), q \in \{-, \cdot,+\}$ & influences that reach a node $v$ at the end of the diffusion\\ \hline
		$k=\sum_{s \in S,c _in C} I(S)[q] \in \{+,-\}$ & Cardinality of the set of seeds  \\ \hline
		$|V_{c}| $ & votes for candidate ${c_i}$ at the beginning \\ \hline
		$ |\bar V_{c}(S,y)|$ & votes for candidate ${c}$ at the end \\ \hline
		$ \chi (S,y)$ & number of nodes $v$ reached by some influence and $\pi_v(1)\neq c_*$\ \\ \hline
		$\mathcal{M}$ & 	change in the margin of victory\\  \hline
		TBR & Tie-breaking rule \\  \hline
	\end{tabular}
	\renewcommand{\arraystretch}{1}
	
	\caption[Symbols' table]{Symbols' table.}
	\label{tab:notation}
\end{table}




	
	
	
	


==> reduction.tex <==
We start
next prove a very general result that relates the possibility of spreading messages such that the candidate 

\subsubsection{Positive Influence Only.}
\begin{theorem}
	 If only positive influence is possible, computing $max_{|S|\le k}\mathcal M(S)$ in elections is not in \PolyAPX.
\end{theorem}

% \begin{proof}
% 	
% 
% \begin{definition}[SET COVER]
% 	Given a finite set $N=\{z_1,\dots,z_n\}$ of elements and a collection $X=\{x_1,..,x_m\}$ of set with $x_i \subseteq N$, is there a collection $X^*\subseteq X$ such that $|X^*|\le h$ and $\cup_{x_i \in X^*}\ x_i= N$?
% \end{definition}
% 
% \textbf{mapping.} 
% %Suppose $h \le m-3$, otherwise the instance is easy(can be solve by enumeration).
% 
% Given a instance of set cover $(N,M,h)$ we construct a graph as follow:
% 
% All edge has probability $1$ (if not differently specified) and can be used  $k=h+1$ seeds.
% The candidates are $C=\{c_*,c_1,c_2\}$.
% 
% For each $z_i \in N$, we add a node $v_{z_i}$ with preferences $\pi_{v_{z_i}}=c_2>c_1>c_*$;
% for each $x_i \in X$, we add a node $v_{x_i}$ with an edge toward each $z \in x_i$  and preferences $\pi_{v_{x_i}}=c_2>c_1>c_*$;
% Let define $G_1=\{V_{z_i}: z_i \in N\} \cup \{V_{x_i} : x_i \in X\}$
% 
% We build two completely connected subgraph $G_2$ with $|G_2|=4(n+m)+m-h-1$ and $G_3$ with $|G_3|=n+h+1$.
% %Each node $v\in G_1$ has a edge to each node in $G_2$.
% %Each node in $v \in G_2$ has preferences $\pi_v=c_1>c_2>c_*$.
% 
% $2(n+m)+m-h-1$ nodes in $G_2$ have preferences $\pi_v=c_1>c_2>c_*$. We define this set of nodes as $G_2^1$.
% 
% $2(n+m)$ nodes in $G_2$ have preferences $\pi_v=c_2>c_1>c_*$. We define this set of nodes as $G_2^2$.
% 
% Each node in $v \in G_3$ has preferences  $\pi_v=c_1>c_2>c_*$.
% 
% We add a graph $G_4$ with $|G_4|=3(n+m)+2$ disconnected nodes with  preferences  $c_*>c_1>c_2$.
% We add two node $v_a$ and $v_b$, an edge from each node in $G_1 \cup G_2 \cup G_3$ to  $v_a$ and $v_b$, and $2$ edges between $v_a$ and $v_b$ with $p_{v_a,v_b}=p_{v_b,v_a}=1-\epsilon$.
% Let $\pi_{v_a}=\pi_{v_b}=c_1>c_2>c_*$.
% 
% Notice that since $ |V_{c_*}|-\max \{ |V_{c_1}|, |\bar V_{c_2}|\}=0$,
% 
%  $\mathcal M(S)=|\bar V_{c_*}(S)|- E_y[\max \{ |\bar V_{c_1}(S,y)| |V_{c_2}(S,y)|\}|]$.
% 
% \textbf{if SET COVER is satisfiable then $\mathcal M(S^*)\ge 1$.}
% 
% If a instance $(N,X,h)$ of SET COVER is satisfiable there exists a set $X^*\subseteq X$  such that $|X^*|\le h$ and $\cup_{x_i \in X^*}=N$ .
%  
% Suppose we choose a node $v \in G_3$ and influence it with $I(v)=(\cdot,\cdot,+)$.
% Moreover, let influence  each voter  $v_{x_i}, x_i \in X^*$, with $I(v_{x_i})=(\cdot,+,\cdot)$.
% 
% At the end of the diffusion $|\bar V_{c_1}(S)|$ = $3(n+m)+1$ ($h+n$ nodes of $G_1$, $2(n+m)+m-h-1$ nodes of $G_2$, $v_a$ and $v_b$).
% 
% At the end of the diffusion $|\bar V_{c_2}(S)|$= $3(n+m)+1$($m-h$ nodes of $G_1$, $2(n+m)$ nodes of $G_2^2$ and $n+h+1$ nodes of $G_3$).
% 
% Thus, $\mathcal M(S)=3(m+n)+2-\max\{|\bar V_{c_1}(S)|,|\bar V_{c_2}(S)|\}=1$.
% 
% 
% \textbf{If  SET COVER is not satisfiable then $\mathcal M(S^*)=\epsilon$.}
% 
% First, we prove that if the only seeds are $I(v_a)=(\cdot,\cdot,+)$ and $I(v_b)=(\cdot,+,\cdot)$, $\mathcal M(S)=\epsilon$.
% Two cases are possible: $y_1$ if edge $(v_b,v_a)$ exists in the live-graph, $y_2$ otherwise.
%  $|\bar V_{c_1}(S,y_1)|=3(n+m)+2$, $|\bar V_{c_2}(S,y_2)|=3(n+m)$,
% $|\bar V_{c_1}(S,y_2)|=3(n+m)+1$, and $|\bar V_{c_2}(S,y_2)|=3(n+m)+1$.
% Thus, $\mathcal M(S)= 3(n+m)+2- [ (1-\epsilon)  max\{|\bar V_{c_1}(S,y_1)|,|\bar V_{c_2}(S,y_1)|\}
% + \epsilon\ max\{|\bar V_{c_1}(S,y_2)|,|\bar V_{c_2}(S,y_2)|\}]=\epsilon.$
% 
% We prove that $MOV(S^*) \le \epsilon$. 
% Notice that $c_*$ cannot increase her votes, since she is always or first or last in the preferences, and each seed has always $I(s) \in (\cdot, \{+,\cdot\}\{+,\cdot\})$.
% 
% 
% 
% %First we prove that if  $I(v_a)\neq (\cdot,\cdot,\cdot)$ or $I(v_b)\neq (\cdot,\cdot,\cdot)$, $\mathcal M(S^*)<\epsilon$.
% 
% %If $ I(v_a)=(\cdot,+,\{+,\cdot\})$ or $I(v_b)=((\cdot,+,\{+,\cdot\})$, all nodes in $G_2^1\cup G_3$ will vote $c_1$ and $|\bar V_{c_1}(S)|\ge m+n+2$ with probability $1-\epsilon$, $|\bar V_{c_1}(S)| \ge m+n+1$ with probability $\epsilon$, and $\mathcal M(S) \le \epsilon$.
% %If $ I(v_a)=(\cdot,\cdot,+)$ and $I(v_b)=(\cdot,\cdot,\cdot)$ (and in the symmetric case), all nodes in $G_1$ will vote $c_2$ and $|\bar V_{c_2}(S)| \ge m+n+1$ with probability $\epsilon$, $|\bar V_{c_2}(S)| \ge m+n+2$ with probability $1-\epsilon$, and $\mathcal M(S) \le \epsilon$.
% %Similarly, if $I(v_a)=(\cdot,\cdot,+)$, $I(v_b)=(\cdot,\cdot,+)$, all nodes in $G_1$ will vote $c_2$ and $|V_{c_2}(S) \ge m+n+2$ and $\mathcal M(S) \le 0$.
% 
% 
% If $\mathcal M(S^*) > \epsilon$,
% $c_2$ must take some of the $c_1$ votes. Thus, or 
% \\$(1)$ $c_2$ gains votes from nodes in $G_2^1$;
% \\$(2)$ $c_2$ gains votes from nodes in $G_3$;
% \\$(3)$  $c_2$ gains votes from nodes in $v_a$ or $v_b$.
% 
% 
% Suppose by contradiction that case $(1)$ is true.
% This implies that $c_2$ take all the votes of $c_1$ in $G_2^1$. It easy to see that in this case $c_2$ cannot loose his initial votes in $G_2^2$, $|\bar V_{c_2}(S)| \ge 4(n+m) +m-h-1$ and $\mathcal M(S)\le 0$. Similarly, can be proved that $c_1$ cannot takes $c_2$ votes in $G_2^2$, $G_2^1$ will vote for $c_1$ and $G_2^2$ will vote for $c_2$.
% 
% Suppose by contradiction that case $(2)$ is true and case $(1)$ is false.
% This implies that exist a node $v_1 \in G_3$ with $I(v_1)=(\cdot,\cdot,+)$ and it does not exist a node $v_2 \in G_3$ with $I(v_2)=(\cdot,+,\{+,\cdot\})$. $|\bar V_{c_2}(S)|$ is greater than the sum of $|G_2^2|$, $|G_3|$ and the node in $v \in G_1$ that do not vote for $c_1$. Let identify $Q$ has the number of nodes $v \in G_1$ with $\bar I(v,S)=(\cdot,+,\cdot)$.
%  $|\bar V_{c_2}(S)| \ge |G_3|+|G_2^2|+|G_1|-|Q|$.
% Since $\mathcal M(S) \le |\bar V_{c_*}(S)|-|\bar V_{c_2}(S)|\le 3(m+n)+2-(|G_3|+|G_2^2|+|G_1|-|Q|)$, $\mathcal M(S) > 0$ implies $|Q| \geq h+n$, that is impossible since $(M,N,h)$ is not satisfiable.
% 
% Suppose by contradiction that case $(3)$ is true and case $(1)$ and $(2)$ are false.
% It must be $\bar I(v_a,S,y)=(\cdot,\cdot,+)$ (or $\bar I(v_b,S,y)=(\cdot,\cdot,+) )$ for some live-graph $y$. This implies that all nodes $v$ in $G_1 \cup G_2^2$ has influence $\bar I(v,S)=(\cdot,\cdot,\{+,\cdot\})$ and will vote for $c_2$. 
% If $I(v_b)=(\cdot,+,\{+,\cdot\})$, candidate $c_1$ has at least $3(n+m)+2$ votes with probability $1-\epsilon$ and $\mathcal M(S) \le 0$.
% if  $I(v_b)=(\cdot,\cdot,\{+,\cdot\})$, candidate $c_2$ has at least $3(n+m)+2$ votes with probability $1-\epsilon$ and $\mathcal M(S) \le 0$.
% 
% 
% \end{proof}

Similar reduction is possible when only negative influence is possible.

\medskip

\begin{theorem}
	If only positive influence is possible, maximizing the probability of victory in elections is not in \PolyAPX.
\end{theorem}

% \begin{figure}
% 	\includegraphics[width=\linewidth]{figures/riduzione3giocatori.pdf}
% 	\caption{reduction for 3 candidates and only positive influence available.}
% 	\label{fig:reductionPositive}
% \end{figure}

% The second variant that we want to analyze concerns the adopted tie-breaking rule. 
If only positive influences propagate, there are no ties that should be evaluated, so the previously obtained results for the standard TBR still hold for both the optimistic and pessimistic TBR.




